Optimal Byzantine Resilient Convergence in Asynchronous Robot Networks

We propose the first deterministic algorithm that tolerates up to $f$ byzantine faults in $3f+1$-sized networks and performs in the asynchronous CORDA model. Our solution matches the previously established lower bound for the semi-synchronous ATOM model on the number of tolerated Byzantine robots. Our algorithm works under bounded scheduling assumptions for oblivious robots moving in a uni-dimensional space.

==> CNS.tex <==
%\section{Preliminaries}
%\label{sec:preliminaries}
\section{The Byzantine Convergence Problem}

\remove{
In the following we refine the definition of the \emph{point convergence problem} from~\cite{agmon2004ftg}: given an initial configuration of $N$ autonomous mobile robots, for every $\epsilon > 0$, there is a time $t_\epsilon$ from which all correct robots are within distance of at most $\epsilon$ of each other.
}

Given an initial configuration of $N$ autonomous mobile robots ($m$ of which are correct such that $m \geq N-f$), the \emph{point convergence problem} requires that all correct
robots asymptotically approach the exact same, but unknown beforehand,
location. In other words, for every $\epsilon > 0$, there is a time $t_\epsilon$ from which all correct robots are within distance of at most $\epsilon$ of each other.

\begin{definition}[Byzantine Convergence]
\label{def:byz-convergence}
A system of oblivious robots verify the Byzantine convergence specification if and only if $\forall \epsilon > 0, \exists t_\epsilon$ such that $\forall t > t_\epsilon$, $\forall$ i,j $\leq m, \mathit{distance}(U_i(t), U_j(t)) < \epsilon$, where $U_i(t)$ and $U_j(t)$ are the positions of some \emph{correct} robots $i$ and $j$ at time $t$, and where $\mathit{distance}(a,b)$ denote the Euclidian distance between two positions. 
\end{definition}

Definition~\ref{def:byz-convergence} requires the convergence property only from the \emph{correct} robots. Note that it is impossible to obtain the convergence of all the robots in the system regardless their behavior since Byzantine robots may exhibit arbitrary behavior and never join the position of correct robots.


In the following we recall the necessary and sufficient conditions to achieve convergence in systems prone to byzantine failures. We first focus on the definition of \emph{shrinking} algorithms (algorithms that eventually decrease the range among correct robots). In \cite{} we proved that this condition is necessary but not sufficient for convergence even in fault-free environments. We then recall the defintion of \emph{cautious} algorithms (algorithms that ensure that the position of correct robots always remains inside the range of the correct robots).  This condition combined with the previous one is sufficient to reach convergence in fault-free systems \cite{}. 
%Moreover, we address the necessary and sufficient conditions for convergence in byzantine-prone environments and show 
%that for the problem to admit solutions additional assumptions (\emph{e.g.} multiplicity knowledge) are necessary.

By definition, convergence aims at asymptotically decreasing the range of possible values for the correct robots. The shrinking property captures this property. An algorithm is shrinking if there exists a constant factor $\alpha \in (0,1)$ such that starting in any configuration the range of correct robots eventually decreases by a multiplicative $\alpha$ factor. 

\begin{definition}\cite{}[Shrinking Algorithm] 
An algorithm is \emph{shrinking} if and only if $\exists \alpha \in (0,1)$ such that $\forall t, \exists t^\prime > t$, such that $diam(U(t^\prime)) < \alpha*diam(U(t))$, where $U(t)$ is the multiset of positions of correct robots.
\end{definition}

%\begin{note}
%Note that the definition does not imply that the diameter always remains smaller than $\alpha*diam(U(t))$ after $t^\prime$. 
%(see Figure~\ref{fig-oscillatory} in the Appendix). 
%Therefore, an oscillatory effect is possible: the algorithm alternates between periods where the diameter is increased and decreased. However, each increasing period is followed by a decreasing one.
% as depicted in Figure~\ref{fig-oscillatory}. 
%Therefore a shrinking algorithm is not necessarily convergent.
%\end{note}

%\begin{lem}
%\label{lem:convergence}
%Any algorithm solving the convergence problem is necessarily shrinking.
%\end{lem}

A natural way to solve convergence is to never let the algorithm increase the diameter of correct robot positions. We say in this case that the algorithm is cautious. This notion was first introduced in~\cite{dolev1986raa}. A cautious algorithm is particularly appealing in the context of byzantine failures since it always instructs a correct robot to move inside the range of the positions held by the correct robots regardless of the locations of Byzantine ones. The following definition introduced first in \cite{} customizes 
the definition of cautious algorithm proposed in \cite{dolev1986raa} to robot networks.

\begin{definition}\cite{}[Cautious Algorithm]
Let $D_i(t)$ the last destination calculated by the robot $i$ before time $t$ and let $U^i(t)$ the positions of the correct robots as seen by robot $i$ before time $t$. \footnote{If the last calculation was executed at time $t^\prime \leq t$ then $D_i(t) = D_i(t^\prime)$.} An algorithm is \emph{cautious} if it meets the following conditions:
\begin{itemize}
\item \textbf{cautiousness: } $\forall t,~D_i(t) \in range(U^i(t))$ for each robot $i$.
\item \textbf{non-triviality: } $\forall t$, if $diameter(U(t)) \neq 0$ then $\exists t^\prime>t$ and a robot $i$ such that $D_i(t^\prime)\neq U_i(t^\prime)$
(at least one correct robot changes its position).
\end{itemize}
\end{definition}

%Note that the non-triviality condition ensures progress. That is, it prevents trivial solutions where each robot stays at its current position forever. 

\remove{
\paragraph{}
The following lemma states an important property of cautious algorithms in the CORDA model. We consider the range of correct robots and their destinations and we prove that this range never decreases if the algorithm is cautious.

\begin{lem}
\label{diam-AS} 
In the CORDA model, if an algorithm is cautious then $ \forall t^\prime > t, diam(U(t)\cup D(t)) \leq diam(U(t^\prime) \cup D(t^\prime))$.
\end{lem}

\begin{proof}
We assume to the contrary that $\exists t^\prime > t$ such that $diam(U(t^\prime) \cup
D(t^\prime)) > diam(U(t) \cup D(t))$, and 
prove that this leads to a contradiction.
Then there exists at least one correct robot, say $r_k$, whose both
position and destination were inside 
$range(U(t) \cup D(t))$ at $t$, and whose position or destination is outside the range at $t^\prime$. 
Formally, there exists some $t^\prime>t$ such that 
$U_k(t^\prime) \notin range(U(t) \cup D(t))$ or $D_k(t^\prime) \notin range(U(t) \cup D(t))$. 

Assume without loss of generality that $r_k$ is the  only robot in this case between $t$ and $t^\prime$, and distinguish the following two cases: 

\begin{enumerate}
\item The destination point of $r_k$ is outside $range(U(t)\cup D(t))$
at $t^\prime$, that is $D_k(t^\prime) \notin
range(U(t)\cup D(t))$. 
But since no other robot was outside the range after t, and since
$D_k(t^\prime)$ was calculated 
after $t$,  $D_k(t^\prime)$ is necessarily inside the range (by the definition of cautious algorithms), which leads to a contradiction.
\item The position of  $r_k$ is outside $range(U(t) \cup D(t))$ at
$t^\prime$, that is $U_k(t^\prime) 
\notin range(U(t)\cup D(t))$. But since both the precedent position of
$r_k$ and its destination point 
were inside $range(U(t)\cup D(t))$, $r_k$ can only move between these
two points and stays necessarily 
inside $range(U(t) \cup D(t))$ which leads to a contradiction.
\end{enumerate}
The two cases lead to a contradiction which proves our lemma.
\end{proof}
}
The following theorem will be further used in order to prove the correctness of our convergence algorithm.

\begin{thm}\cite{}
\label{lem:cands}
Any algorithm that is both cautious and shrinking solves the convergence problem in fault-free robot networks.
\end{thm}

 


==> annexes.tex <==
\newpage
\section*{Appendix}

%***************************   Multiplicity and multiples detection *********************%


\subsection*{Necessary and sufficient conditions for convergence}

\begin{figure}[htbp]
\begin{center}
\includegraphics[height=6cm]{Diagramme4.eps}
\caption{Oscillatory effect of a shrinking algorithm}
\label{fig-oscillatory}
\end{center}
\end{figure}

\begin{lem-repeat}{lem:convergence}
Any algorithm solving the convergence problem is necessarily shrinking.
\end{lem-repeat}

\begin{proof}
Assume that a convergence algorithm is not shrinking.
Then there exists some constant factor $\alpha \in (0,1)$, and some
time instant $t_1$ such that 
the diameter of correct robots after $t_1$ never decreases by a factor
of $\alpha$ i.e. 
$diam(U(t_2))$ is greater than $\alpha*diam(U(t_1))$ for any $t_2 > t_1$.
Therefore, there will always exist two correct robots that are at
distance of at least 
$\alpha*diam(U(t_1))$, which contradicts the assumption that the algorithm is convergent.
\end{proof}

\begin{lem-repeat}{diam-SS} 
In the ATOM model, if an algorithm is cautious then $\forall t^\prime >t~ diam(U(t^\prime)) \leq diam(U(t))$.
\end{lem-repeat}

\begin{proof}
Assume that it is not the case. i.e. that
$diam(U(t^\prime))>diam(U(t))$ for some $t^\prime>t$. Then there
exists two 
\textbf{successive} time instants, referred in the following cycles, $t_2>t_1$ such that $t\leq
t_1<t^\prime$,  $t<t_2 \leq t^\prime$ and 
the diameter of correct robots at $t_2$ is strictly greater than the diameter at $t_1$ i.e. $diam(U(t_2))>diam(U(t_1))$.
Thus, there exists at least one correct robot, say $r_1$, that was
inside $range(U(t_1))$ at $t_1$, 
and moved outside it at $t_2$. We prove that this is impossible.

Since cycles are atomic, no robot can move between $t_1$ and the LOOK
step of $t_2$, and the resulting 
snapshot of correct robots at this step is equal to $U(t_1)$. 
Thus, the destination point calculated by $r_1$ at $t_2$ is
necessarily inside $range(U(t_1))$ since the algorithm is cautious.

This contradicts the assumption that $r_1$ moves outside $range(U(t_1))$ at $t_2$, and the lemma follows.
\end{proof}

\begin{lem-repeat}{diam-AS} 
In the CORDA model, if an algorithm is cautious then $ \forall t^\prime > t, diam(U(t)\cup D(t)) \leq diam(U(t^\prime) \cup D(t^\prime))$.
\end{lem-repeat}

\begin{proof}
We assume that $\exists t^\prime > t$ such that $diam(U(t^\prime) \cup
D(t^\prime)) > diam(U(t) \cup D(t))$, and 
prove that this leads to a contradiction.
Then there exists at least one correct robot, say $r_k$, whose both
position and destination were inside 
$range(U(t) \cup D(t))$ at $t$, and whose position or destination is outside the range at $t^\prime$. 
Formally, there exists some $t^\prime>t$ such that 
$U_k(t^\prime) \notin range(U(t) \cup D(t))$ or $D_k(t^\prime) \notin range(U(t) \cup D(t))$. 

Assume without loss of generality that $r_k$ is the  only robot in this case between $t$ and $t^\prime$, and distinguish the following two cases: 

\begin{enumerate}
\item The destination point of $r_k$ is outside $range(U(t)\cup D(t))$
at $t^\prime$, that is $D_k(t^\prime) \notin
range(U(t)\cup D(t))$. 
But since no other robot was outside the range after t, and since
$D_k(t^\prime)$ was calculated 
after $t$,  $D_k(t^\prime)$ is necessarily inside the range (by the definition of cautious algorithms), which leads to a contradiction.
\item The position of  $r_k$ is outside $range(U(t) \cup D(t))$ at
$t^\prime$, that is $U_k(t^\prime) 
\notin range(U(t)\cup D(t))$. But since both the precedent position of
$r_k$ and its destination point 
were inside $range(U(t)\cup D(t))$, $r_k$ can only move between these
two points and stays necessarily 
inside $range(U(t) \cup D(t))$ which leads to a contradiction.
\end{enumerate}
The two cases lead to a contradiction which proves our lemma.
\end{proof}



\begin{lem-repeat}{lem:cands}
Any algorithm that is both cautious and shrinking solves the convergence problem in fault-free robot networks.
\end{lem-repeat}

\begin{proof}
We construct our proof for the most general model (the CORDA model).
Since the algorithm is shrinking then:
$\exists \alpha \in (0,1)$ such that $\forall t$, there exists some time
$t^\prime> t$, 
such that $diam(U(t^\prime) < diam(U(t))*\alpha$ and then $diam(U(t^\prime) \cup D(t^\prime)) < diam(U(t) \cup D(t))*\alpha$.
And since it is cautious, we have by Lemma \ref{diam-AS} that
$diam(U(t) \cup D(t)) \leq diam(U(t^\prime) \cup D(t^\prime)) \forall t^\prime > t$.
So $\exists \alpha \in (0,1)$ such that $\forall t$, there exists some time $t^\prime > t$, such that \textbf{$\forall t^{\prime\prime} >t^\prime$},
$diam(U(t^{\prime\prime})\cup D(t^{\prime\prime}))<diam(U(t)\cup D(t))*\alpha$.

So given any initial configuration, by recursively decreasing the diameter of correct robots by a factor of $\alpha$, we can make them as close as we like.
Formally speaking, 
if we refer to $diam(U(0)\cup D(0))$ by $\sigma_0$ (the initial range), then for every $\epsilon > 0$,
there exists $k>0$, so that  ${s\sigma_0}/{\alpha^k} < \epsilon$, 
and the algorithm is convergent.
\end{proof}

\begin{lem-repeat}{lem:nec}
It is impossible to reach convergence with a cautious algorithm in Byzantine-prone environments without additional assumptions, even in the presence of a single Byzantine fault.
\end{lem-repeat}

\begin{proof}
Let $A$ and $B$ be two distinct points in a uni-dimensional space (see
Figure \ref{fig-multiplicity-necessary}), 
and consider a set of robots without any multiplicity detection
capability. We suppose that it is possible to achieve convergence in
this case in presence of a 
single byzantine robot and we show that this leads to a contradiction.



\begin{figure}[htbp]
\begin{center}
\includegraphics[width=7cm]{Diagramme1.eps}
\caption{Necessity of multiplicity detection to achieve convergence (black robots are byzantine)}
\label{fig-multiplicity-necessary}
\includegraphics[width=7cm]{Diagramme2.eps}
\caption{Necessity of multiplicity number detection to achieve convergence (black robots are byzantine)}
\label{fig-multiplicity-nb-necessary}
\end{center}
\end{figure}


\begin{enumerate}
\item Let $C_1$ be a configuration where all correct robots are at $A$, and one byzantine robot at $B$.
If the robots at $A$ move, the scheduler can stop them at different
locations which causes the diameter of 
correct robots to increase which contradicts Lemma~\ref{diam-SS}, so they must stay at $A$.
\item Similarly, let $C_2$ be the symmetric configuration where the byzantine robot is at $A$, and the correct ones at $B$.  Then the robots at $B$ cannot move.
\item Let $C_3$ be a configuration where correct robots are spread over $A$ and $B$.  the byzantine robot may be indifferently at $A$ or at $B$. 
Since the robots are not endowed with a multiplicity detection
capability, the configurations $C_1$, $C_2$ and $C_3$ 
are indistinguishable to them. So they stay at their locations and the
algorithm never converge 
which contradicts the assumption that convergence is possible in this case.
\end{enumerate}
This proves that at least a simple multiplicity detector is necessary
to achieve convergence even if a single robot 
is byzantine.
\end{proof}


\begin{lem-repeat}{lem:suff}
The necessary and sufficient condition to reach Byzantine-tolerant convergence in a uni-dimensional space via cautious algorithms is multiples detection.
\end{lem-repeat}

\begin{proof}
The Algorithm \ref{alg:1} is a cautious algorithm that converges under
the assumption of multiples detection.
The previous lemma show that convergence cannot be achieved without
additional assumptions. Hence we consider the minimal set of
assumptions: robots are endowed with a simple multiplicity detection.
In the following we assume that convergence can be achieved with only 
simple multiplicity detection and we show that this leads to a contradiction.
Consider a set of robots in a uni-dimensional space prone to byzantine
failures and endowed 
with simple multiplicity detectors. The robots are spread over two
distinct points of the uni-dimensional 
space $A$ and $B$ (see figure \ref{fig-multiplicity-nb-necessary}).
\begin{enumerate}
\item Let $C_1$ be a configuration where all correct robots are at $A$,
and byzantine ones at $B$.  
We suppose that the number of correct robots at $A$ is sufficiently large to tolerate the byzantine robots of $B$. 
If the robots at $A$ move, they may be stopped by the scheduler at
different locations which increase their diameter. This contradicts
Lemma~\ref{diam-SS} because 
the algorithm is cautious. So the correct robots stay at $A$.
\item Consider the symmetric configuration $C_2$ where the correct
robots are at $B$ and 
the byzantine ones at $A$. With the same argument as $C_1$ we find that robots at $B$ stay there.
\item Let $C_3$ be a configuration where correct and byzantine robots are spread evenly between $A$ and $B$. 
Since robots are endowed only with simple multiplicity detectors, the
configurations $C_1$, $C_2$ and $C_3$ are indistinguishable to
them. So no 
robot will move and the algorithm never converges. This proves the lemma. 
\end{enumerate}
\end{proof}

\subsection*{Lower bounds}
\begin{lem-repeat}{lem:lb}
Byzantine-resilient convergence is impossible for $n \leq 3f$ with a cautious algorithm in the semi-synchronous ATOM model.
\end{lem-repeat}

\begin{proof}
By Lemma \ref{impossibility-2f}, convergence is impossible for $n \leq
2f$ in the fully-synchronous ATOM model, so it is also impossible in the semi-synchronous case.
Assume that there exists a cautious algorithm that achieves
convergence with $2f < n \leq 3f$.

Let A and B be two distinct points in a uni-dimensional space such that $(n-f)$ robots are located at A 
%and their positive direction(orientation?) is towards B. 
and the remaining f robots are located at B (see Figure \ref{fig-impossibility-3f} for $n=6$ and $f=2$).
%and their positive direction is toward A.

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=7cm]{Diagramme5.eps}
\caption{Impossibility of convergence in SYM with $n\leq 3f$, black robots are byzantine}
\label{fig-impossibility-3f}
\end{center}
\end{figure}

Let $C_1$ be a configuration where all correct robots are at A and the byzantine ones at B. Note that since the correct robots are at the same point, the diameter is 0.
There are two possible cases:

a)The robots at A move when activated: since the algorithm is cautious, the only possible direction is towards B. 
When moving towards B, the robots may be stopped by the scheduler at different locations which causes the diameter to increase and this contradicts Lemma \ref{diam-SS}.

b)The robots at A do not move: the only possible action for robots in this configuration since they cannot move.

Let $C_2$ be another possible configuration where the byzantine robots are at A, and the correct ones are spread over A and B as follows: $f$ correct robots at B and the remaining $(n-2f)$ at A.

 Note that $C_1$ and $C_2$ are indistinguishable by the individual robots
and assume the following scenario: The scheduler activates robots at
A. Since the configurations $C_1$ and $C_2$ are equivalent, robots
at A do not move. Then, the scheduler moves $n-2f \leq f$ faulty
robots from A to B which leads to the symmetric 
configuration $C_2^\prime$ and robots at B do not move neither. The
same scenario is repeated 
infinitely and no robot will ever move which prevents the algorithm to converge.
%\\note: j'ai fait la preuve sur la non convergence pour un cautious, j'aurai d%u la faire pour non shrinkingness pour un cautious ?
\end{proof}




\subsection*{Properties of Algorithm \ref{alg:1}}
\begin{lem-repeat}{inside_range}
For Algorithm \ref{alg:1} and for $n>3f$, $range(trim_f(U(t))) \subseteq  range(trim_f(P(t)))$.
\end{lem-repeat}

\begin{proof}
We prove that: 
\begin{enumerate}
\item $\forall t~ U_{f+1}(t) \in range(trim_f(P(t))).$
\item $\forall t~ U_{m-f}(t) \in range(trim_f(P(t))).$
\end{enumerate}

\begin{enumerate}
\item 
Suppose that $U_{f+1}(t) \notin range(trim_f(P(t)))$. Then either $U_{f+1}(t) < \min(trim_f(P(t)))$ or $U_{f+1}(t) > \max(trim_f(P(t)))$.

\begin{itemize}

\item If $U_{f+1}(t) < \min(trim_f(P(t)))$ then there are at least $f+1$ positions ($U_1(t), ..., U_{f+1}(t)$) which are smaller than $\min(trim_f(P(t)))$. This contradicts the definition of $trim_f(P(t))$ (only the $f$ smallest and the $f$ largest elements of P(t) are removed). 

\item If $U_{f+1}(t) > \max(trim_f(P(t)))$ and since $|U(t)| > 2f$ (because $n>3f$), then there are also at least $f+1$ positions in U(t) greater than $\max(trim_f(P(t)))$, which leads to a contradiction.

\end{itemize}

\item The property is symmetric the precedent one.
\end{enumerate}
\end{proof}



\begin{lem-repeat}{destination_mid}
For Algorithm~\ref{alg:1} and for $n>3f$, we have the following properties:
\begin{enumerate}
\item $\forall i,~\forall t~ D_i(t) \leq (U_{f+1}(t) + U_m(t))/2.$
\item $\forall i,~\forall t~ D_i(t) \geq (U_1(t) + U_{m-f}(t))/2.$
\end{enumerate}
%//si je pose que n' est le nombre total de robots. les 2 lemmas reste valables pour u1+(n'-2f)
\end{lem-repeat}

\begin{proof}

Take $d_1$ to be the distance between $U_{f+1}(t)$ and $U_m(t)$.
\begin{enumerate}
\item 
Suppose $D_i(t) > (U_{f+1}(t) + U_m(t))/2$ for some correct robot $i$ at time $t$. 
Then $U_{f+1}(t) < D_i(t)-d_1/2$. And by Lemma~\ref{inside_range}, $U_{f+1}$(t) is inside $range(trim_f(P(t)))$ which means that there is a position inside $range(trim_f(P(t)))$ which is smaller than $D_i(t)-d_1/2$.
Hence there must exists a position inside $range(trim_f(P(t)))$, say p, which is greater than $D_i(t)+d_1/2$ because $D_i$ is the mean of $trim_f(P(t))$. 

$p > D_i(t)+d_1/2$ implies that $p>U_m(t)$, and by lemma~\ref{range-trim} $U_m(t) \geq \max(range(trim_f(P(t))))$ so $p>\max((trim_f(P(t)))$ which contradicts the fact that p is inside $range(trim_f(P(t)))$.

\item Symmetric to the precedent property.
\end{enumerate}

\end{proof}


\begin{lem-repeat}{uf-less-st}
Let $S(t)$ be a multiset of $f+1$ arbitrary elements of U(t). We have the following properties:
\begin{enumerate}
\item $\forall t~ U_{f+1}(t) \leq \max(S(t))$
\item $\forall t~ U_{m-f}(t) \geq \min(S(t))$
\end{enumerate}
\end{lem-repeat}

\begin{proof}
\begin{enumerate}
\item Assume to the contrary that $U_{f+1}(t) > \max(S(t))$. This means that $U_{f+1}(t)$ is strictly greater than at least $f+1$ elements of U(t), which leads to a contradiction.
\item The property is symmetric to the precedent.
\end{enumerate}
\end{proof}
 
 
 
\begin{lem-repeat}{limit-destinations}
Let a time $t_2>t_1$ and let $S(t)$ be a multiset of $f+1$ arbitrary elements in U(t).
If all the values of $S(t)$ between $t_1$ and $t_2$ are smaller than
some value $S_{max}$, then all the destination 
points calculated by elements of $U(t)$ between $t_1$ and $t_2$ are smaller or equal to $S_{max}+U_m(t_1)/2$.
Formally, if $\forall p \in S(t)$ and  $\forall t \in [t_1, t_2]~ p \leq S_{max}$  
then for each correct robot i in $U(t)$ and for each $t \in [t_1, t_2]~ D_i(t) \leq (S_{max}+U_m(t_1))/2$.
\end{lem-repeat}

\begin{proof}
By definition of $S_{max}$ we have that $\forall t \in [t_1, t_2], max(S(t)) \leq S_{max}$.
According to Lemma~\ref{uf-less-st}, $\forall t \in [t_1, t_2]~  U_{f+1}(t) \leq max(S(t))$. 
So $\forall t \in [t_1, t_2]~ U_{f+1}(t) \leq S_{max}$.

By Lemma~\ref{destination_mid}, for each correct robot i and for each $t  \in [t_1, t_2] $, $D_i(t) \leq (U_m(t) + U_{f+1}(t))/2$. 
So for each correct robot i and for each $t  \in [t_1, t_2]$, $D_i(t) \leq (U_m(t)+S_{max})$ .
Since the algorithm is cautious, $ \forall t  \in [t_1, t_2]~ U_m(t) \leq U_m(t_1) $ and the lemma follows.

\end{proof}

\subsection*{Convergence of Algorithm \ref{alg:1} in fully-synchronous
ATOM model}

In this section we address the correctness of Algorithm \ref{alg:1} in
the fully-synchronous ATOM model.


\begin{lem}
\label{shrinking-FS}
Algorithm \ref{alg:1} is shrinking for $n>2f$ in fully-synchronous ATOM model.
\end{lem}

\begin{proof}
Let a configuration of robots at time $t$, and let $d_t$ 
be the diameter of correct robots at $t$.
Each cycle, all robots move towards the same destination. They move by
at least a distance of $\delta$ unless they reach their destination.

If all robots are at a distance smaller than $\delta$ from the common
destination point, 
gathering is achieved and the diameter is null. Otherwise, the robots
that are further than $\delta$ from the destination point approach it
by at least $\delta$ so the diameter decreases by at least $\delta$.
Overall, the diameter of robots decreases by at least factor of 
$\alpha=1-(\delta/d_t)$ at each cycle and thus the algorithm is shrinking.
\end{proof}


The correctness of Algorithm \ref{alg:1} follows directly from Lemma \ref{cautious-FS} and Lemma \ref{shrinking-FS}:

\begin{thm}
Algorithm \ref{alg:1} is convergent for $n>2f$ in fully-synchronous ATOM model.
\end{thm}



\subsection*{Impossibility of convergence of Algorithm \ref{alg:1}
under an arbitrary fair scheduler}
\begin{lem}
\label{lemma:imp}
Algorithm \ref{alg:1} is not convergent in ATOM model in systems with
$n>3f$ even if the arbitrary scheduler is fair.
\end{lem}



\begin{proof}
%prkoi des ri au lieu des pi(t) !\\
%We construct the following scenario:

Let  $U_1(t_0),..., U_m(t_0)$ to be a configuration of correct robots at some initial instant $t_0$.
Assume that they are ordered from left to right, and that their initial diameter is $d_0$.
Note that if at some time $t$, all the byzantine robots are at the
right of correct robots, 
$trim_f(P(t))$ contains the correct positions $U_{f+1}(t),...,
U_m(t)$. And in the case where 
the byzantine robots are to the left of correct robots, $trim_f(P(t))$ contains the correct positions $U_1(t),..., U_{m-f}$.



So, to prevent convergence, the adversary follows the following scenario:
\begin{enumerate}
\item Fix $d$ to be a very small distance compared to $d_0$, for example $d=d_0/100$.

\item The adversary instructs all byzantine robots to move to the right
of the correct robots. Hence $trim_f(P(t_0))$ contains the correct positions $U_{f+1}(t_0), ..., U_m(t_0)$.

\item At $t_1$, the adversary activates simultaneously
the correct robots at $U_{f+1}(t_0),..., U_{m-1}(t_0)$ which move towards $median(trim_f(P(t_0)))$ i.e. the point at the middle between $U_{f+1}(t_0)$ and $U_m(t_0)$. This causes the distance between $U_{f+1}(t_1)$ and $U_m(t_1)$ to decrease by half its initial value at $t_0$ ($distance(U_{f+1}(t_1), U_m(t_1)) = distance(U_{f+1}(t_0), U_m(t_0))/2 $) .

Hence, by repeated application of the same step, the adversary 
can divide this distance by 2 an infinite number of times.

\item Let $t_2$ to be the instant at which $distance(U_{f+1}(t_2), U_m(t_2)) = d$. Then at $t_2$, the adversary activates the robot at $U_m(t_2)$ ($U_m(t_2) = U_m(t_0)$ since the correspondent robot has not been activated between $t_0$ and $t_2$). 

The calculated destination point by the activated robot is $median(U_{f+1}(t_2), U_m(t_2))$ which is at distance $d/2$ from $U_m(t_2)$. Hence the diameter of correct robots decreases by a distance of $d/2$.

\item Then the adversary instructs all the byzantine robots to move to the left of correct robots. And with the same technique as in steps 3 and 4, by activating this time the robots at $U_2(t_2), ..., U_{m-f}(t_2)$ repeatedly, at some time $t_3$, $distance(U_{1}(t_3), U_{m-f}(t_3))$ will be equal to $d$. Then the adversary activates the robot at $U_1(t_3)$ (Note that $U_1(t_3)=U_1(t_0)$) which moves by a distance of $d/2$.

\item At this step, the diameter of correct robots has decreased by a distance of $d$ and all robots have been activated at least once which ensures the fairness of the scheduler. Let $d=d/2$, $t_0=t_3$ and go to step 2.
\end{enumerate}

It follows that the diameter of correct robots will always be greater
than ($d_0-2*d_0/100=(49*d_0)/50$) hence the algorithm is not convergent.
\end{proof}


==> lower_bounds.tex <==
\subsection{Lower bound for byzantine resilient convergence}
\label{sec:lower-bounds}

The following lemma shows that any cautious algorithm needs at least $3f+1$ robots in order to tolerate $f$ byzantine robots in uni-dimensional environments.

\begin{lem}
\label{impossibility-3f-atom}
It is impossible to achieve convergence with a cautious algorithm if $n\leq 3f$ in the ATOM model, where $n$ denotes the number of robots and $f$ denotes the number of Byzantine robots.
\end{lem}

The following corollary provides the lower bound for the CORDA model. 

\begin{cor}
\label{impossibility-3f-corda}
Byzantine-resilient convergence is impossible for $n \leq 3f$ with a cautious algorithm in the CORDA model.
\end{cor}

The following section proves that this bound is tight, the proof is constructive: we give a cautious convergence algorithm that operates correctly in the presence of up to $f$ Byzantine robots provided that the total number of robots is at least $3f+1$, and then we formally prove its correctness.





